Lock-Free Locks Revisited

This paper presents a new and practical approach to lock-free locks based on helping, which allows the user to write code using fine-grained locks, but run it in a lock-free manner. Although lock-free locks have been suggested in the past, they are widely viewed as impractical, have some key limitations, and, as far as we know, have never been implemented. The paper presents some key techniques that make lock-free locks practical and more general. The most important technique is an approach to idempotence -- i.e. making code that runs multiple times appear as if it ran once. The idea is based on using a shared log among processes running the same protected code. Importantly, the approach can be library based, requiring very little if any change to standard code -- code just needs to use the idempotent versions of memory operations (load, store, LL/SC, allocation, free). We have implemented a C++ library called Flock based on the ideas. Flock allows lock-based data structures to run in either lock-free or blocking (traditional locks) mode. We implemented a variety of tree and list-based data structures with Flock and compare the performance of the lock-free and blocking modes under a variety of workloads. The lock-free mode is almost as fast as blocking mode under almost all workloads, and significantly faster when threads are oversubscribed (more threads than processors). We also compare with several existing lock-based and lock-free alternatives.

==> artifact-instructions.tex <==
% !TEX root =  main.tex

\section{Artifact Evaluation Appendix}
\label{sec:ae}

\subsection{Abstract}

This artifact contains the source code and scripts to reproduce all the graphs in Section \ref{sec:exp}.
It includes an implementation of the \flock{} library described in Section~\ref{sec:imp} as well as all the data structures described in Section~\ref{sec:ds}.

\subsection{Artifact check-list (meta-information)}

\begin{itemize}
	\item \textbf{Algorithm:} \flock{} library plus the optimistic fine-grained locking data structures described in Section~\ref{sec:ds}.
	\item \textbf{Program:} microbenchmarks
	\item \textbf{Compilation:} g++ 9.3.0
	\item \textbf{Binary:} binary not included
	\item \textbf{Run-time environment:} Ubuntu 16.04.6 LTS
	\item \textbf{Hardware:} Multi-core machine, preferably with at least 64 logical cores
	\item \textbf{Output:} graphs from Section \ref{sec:exp} as PNG files.
	\item \textbf{Experiments workflow:} one script for compiling the experiments and one script for generating all the graphs.
	\item \textbf{Disk space required (approximately):} 60 MB
	\item \textbf{Time needed to prepare workflow:} approximately 5 minutes
	\item \textbf{Time needed to complete experiments:} approximately 6 hours
	\item \textbf{Publicly available:} yes
	\item \textbf{Code licenses:} MIT License
\end{itemize}

\subsection{Description}

\subsubsection{How delivered}

Available as open source in the \texttt{ae} branch of the following GitHub repository: \url{https://github.com/cmuparlay/flock}.

\subsubsection{Hardware dependencies}

To accurately reproduce our experimental results, a multi-core machine with at least 64 logical cores is recommended.

\subsubsection{Software dependencies}

Our artifact is expected to run correctly under a variety of Linux x86\_64 distributions. Our experiments were compiled using g++ 9.
For scalable memory allocation in C++, we used jemalloc 5.2.1 (\url{https://github.com/jemalloc/jemalloc/releases/download/5.2.1/jemalloc-5.2.1.tar.bz2}) as well as the ParlayLib memory allocator, which is included with the artifact.
Our scripts for running experiments and drawing graphs require a Python 3 installation with mathplotlib.
We used the \texttt{numactl} command to evenly interleave memory across the NUMA nodes.

\subsubsection{Data sets}

None.

\subsection{Installation}

Source code can be complied by running \texttt{bash compile\_all.sh}.

\subsection{Experiment workflow}

After compiling, run \texttt{./generate\_graphs\_from\_paper.sh}  to generate all the graphs and store them in the \texttt{graphs/} directory.

\subsection{Evaluation and expected results}

On a machine with 140 or more logical cores, the results should be very similar to those reported in this paper. 
%This means that if a thread is swapped out while it is in the middle of a range query, no garbage can be collected until it that thread is scheduled again.

\subsection{Experiment customization}

For instructions on how to customize the number of threads, workload, and data structure size in each experiment, please see the README file in the \texttt{ae} branch of the GitHub repository (\url{https://github.com/cmuparlay/flock}).

\subsection{Notes}

None.

\subsection{Methodology}
Submission, reviewing and badging methodology:
\begin{itemize}
	\item \url{https://ctuning.org/ae/submission-20190109.html}
	\item \url{https://ctuning.org/ae/reviewing-20190109.html}
	\item \url{https://www.acm.org/publications/policies/artifact-review-badging}
\end{itemize}

==> biblio.tex <==
@inproceedings{barnes1993method,
  title={A method for implementing lock-free shared-data structures},
  author={Barnes, Greg},
  booktitle=spaa,
  pages={261--270},
  year={1993}
}

@inproceedings{turek1992locking,
	title={Locking without blocking: making lock based concurrent data structure algorithms nonblocking},
	author={Turek, John and Shasha, Dennis and Prakash, Sundeep},
	booktitle=pods,
	pages={212--222},
	year={1992}
}

@article{shavit1997software,
	title={Software transactional memory},
	author={Shavit, Nir and Touitou, Dan},
	journal={Distributed Computing},
	volume={10},
	number={2},
	pages={99--116},
	year={1997},
	publisher={Springer}
}

@article{fraser2007concurrent,
	title={Concurrent programming without locks},
	author={Fraser, Keir and Harris, Tim},
	journal={ACM Transactions on Computer Systems (TOCS)},
	volume={25},
	number={2},
	pages={5--es},
	year={2007},
	publisher={ACM New York, NY, USA}
}

@inproceedings{afek1995wait,
	title={Wait-free made fast},
	author={Afek, Yehuda and Dauber, Dalia and Touitou, Dan},
	booktitle=stoc,
	pages={538--547},
	year={1995}
}

@inproceedings{ben2019delay,
	title={Delay-free concurrency on faulty persistent memory},
	author={Ben-David, Naama and Blelloch, Guy E and Friedman, Michal and Wei, Yuanhao},
	booktitle=spaa,
	pages={253--264},
	year={2019}
}

==> list-experiments.tex <==
\section{Linked List Experiments}

%% list experiments %%
\begin{figure}
	\centering
	\begin{subfigure}{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{graphs/lists_legend.pdf}
	\end{subfigure}
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{graphs/lists-144th-5up-075alpha.pdf}
		\captionsetup{justification=centering}
		\caption{144 th., 5\% up., $\alpha = 0.75$}\label{subfig:list-sizes}
	\end{subfigure}
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{graphs/lists-5up-100size-075alpha.pdf}
		\captionsetup{justification=centering}
		\caption{100 keys, 5\% up., $\alpha = 0.75$}\label{subfig:list-threads}
	\end{subfigure}
	\caption{Throughput of singly and doubly-linked lists.}
	\label{fig:list-exp}
\end{figure}

Experimental results for doubly and singly linked lists can be found in Figure~\ref{fig:list-exp}.
\op{harris\_list} represents Harris's lock-free linked list~\cite{harris2001pragmatic}, and \op{harris\_list\_opt} represents an optimized version where \op{find} operations do not perform any helping~\cite{david2015asynchronized}.



==> lock-proof.tex <==
\section{Proof of Theorem~\ref{theorem:lockfree}}

\begin{proof}
A \emph{helping chain} is the nested sequence of \trylock{}s that a process helps.  In particular when first helping we add the helped \trylock{} to the head of the chain, and if while helping the process recursively helps, it is added to the end of the chain.  We say a \trylock{} helps another if either is runs it in line~\ref{line:help} or it succeeds in the test in line~\ref{line:checklock}, but fails in the test on line~\ref{line:rereadlock} lock.  In the second case the \trylock{} is said to help the last \trylock{} on the lock when failing on the test on line~\ref{line:rereadlock}.  Note that this last \trylock{} will enter after test on line~\ref{line:checklock} and complete before exiting since it will be unlocked when exiting.
\Hao{it actually enters after the read on line 9}
Also note that a \trylock{} will either succeed or add one more to its helping chain.

A helping chain cannot contain two \trylock{}s with the same owner.  This follows from the fact the precedence graph on the locks is lock-cycle free
\Hao{double check}
, and due to idempotence the helper and the helpee must follow the same path of helping.  Since either the helper or helpee could stall at any point, neither can quit early.  Therefore once a \trylock{} initiated by a particular process $p$ is reached by a process $p'$ while helping, either $p$ completes its attempt and all its helping before $p'$ does, in which case $p'$ will just follow $p$'s path doing the same thing, or $p$ completes after in which case $p'$ will never need to help $p$ again since $p$ is busy \Hao{double check}.  In the first case seeing the same process again would imply a cycle in the precedence graph.  This shows $p'$ will only help at most one \trylock{} owned by each other process.   Hence the helping chain has length bounded by $p$, and its step count is bounded by $O(p \tau)$.

Furthermore note that the last \trylock{} in a helping chain must complete an embedded (nested) leaf \trylock{} since otherwise it would fail on a lock and add one more to its helping chain, a contradiction.    Therefore each root \trylock{} is responsible for completing a leaf \trylock, however there is the potential for double counting (e.g. two root \trylock{}s on the same process could be responsible for completing the same leaf \trylock{}).    We note that when done with a helping chain all \trylock{}s on
it have exited (since we remove the locks when done helping).   Therefore the only processes that could follow part of the same chain are ones that have started before the helping chain is done.   There can only be $p-1$ such processes so only that many
can be responsible for completing the same leaf \trylock{}.
This shows that every at most $p$ root \trylock{}s completes a unique leaf \trylock{}.
\end{proof}

